Memorizing Documents with Guidance in Large Language Models

Training data plays a pivotal role in AI models. Large language models (LLMs) are trained with massive amounts of documents, and their parameters hold document-related contents. Recently, several studies identified content-specific locations in LLMs by examining the parameters. Instead of the post hoc interpretation, we propose another approach. We propose document-wise memory architecture to track document memories in training. The proposed architecture maps document representations to memory entries, which softly mask memories in the forward process of LLMs. Additionally, we propose document guidance loss, which increases the likelihood of text with document memories and reduces the likelihood of the text with the memories of other documents. Experimental results on Wikitext-103-v1 with Pythia-1B show that the proposed methods provide different memory entries for documents and high recall of document-related content in generation with trained document-wise memories.

==> ijcai24 <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Biderman \bgroup \em et al.\egroup
  }{2023}]{biderman2023pythia}
Stella Biderman, Hailey Schoelkopf, Quentin~Gregory Anthony, Herbie Bradley,
  Kyle O’Brien, Eric Hallahan, Mohammad~Aflah Khan, Shivanshu Purohit,
  USVSN~Sai Prashanth, Edward Raff, et~al.
\newblock Pythia: A suite for analyzing large language models across training
  and scaling.
\newblock In {\em International Conference on Machine Learning}. PMLR, 2023.

\bibitem[\protect\citeauthoryear{Bills \bgroup \em et al.\egroup
  }{2023}]{bills2023language}
Steven Bills, Nick Cammarata, Dan Mossing, Henk Tillman, Leo Gao, Gabriel Goh,
  Ilya Sutskever, Jan Leike, Jeff Wu, and William Saunders.
\newblock Language models can explain neurons in language models.
\newblock
  \url{https://openaipublic.blob.core.windows.net/neuron-explainer/paper/index.html},
  2023.

\bibitem[\protect\citeauthoryear{Bricken \bgroup \em et al.\egroup
  }{2023}]{bricken2023towards}
Trenton Bricken, Adly Templeton, Joshua Batson, Brian Chen, Adam Jermyn, Tom
  Conerly, Nick Turner, Cem Anil, Carson Denison, Amanda Askell, et~al.
\newblock Towards monosemanticity: Decomposing language models with dictionary
  learning.
\newblock {\em Transformer Circuits Thread}, 2023.

\bibitem[\protect\citeauthoryear{Brown \bgroup \em et al.\egroup
  }{2020}]{brown2020language}
Tom Brown, Benjamin Mann, Nick Ryder, Melanie Subbiah, Jared~D Kaplan, Prafulla
  Dhariwal, Arvind Neelakantan, Pranav Shyam, Girish Sastry, Amanda Askell,
  Sandhini Agarwal, Ariel Herbert-Voss, Gretchen Krueger, Tom Henighan, Rewon
  Child, Aditya Ramesh, Daniel Ziegler, Jeffrey Wu, Clemens Winter, Chris
  Hesse, Mark Chen, Eric Sigler, Mateusz Litwin, Scott Gray, Benjamin Chess,
  Jack Clark, Christopher Berner, Sam McCandlish, Alec Radford, Ilya Sutskever,
  and Dario Amodei.
\newblock Language models are few-shot learners.
\newblock In {\em Advances in Neural Information Processing Systems}, 2020.

\bibitem[\protect\citeauthoryear{Dai \bgroup \em et al.\egroup
  }{2022}]{dai2022knowledge}
Damai Dai, Li~Dong, Yaru Hao, Zhifang Sui, Baobao Chang, and Furu Wei.
\newblock Knowledge neurons in pretrained transformers.
\newblock In {\em Proceedings of the Annual Meeting of the Association for
  Computational Linguistics}, 2022.

\bibitem[\protect\citeauthoryear{Dave \bgroup \em et al.\egroup
  }{2023}]{dave2023chatgpt}
Tirth Dave, Sai~Anirudh Athaluri, and Satyam Singh.
\newblock Chatgpt in medicine: an overview of its applications, advantages,
  limitations, future prospects, and ethical considerations.
\newblock {\em Frontiers in Artificial Intelligence}, 2023.

\bibitem[\protect\citeauthoryear{Dhariwal and
  Nichol}{2021}]{dhariwal2021diffusion}
Prafulla Dhariwal and Alexander Nichol.
\newblock Diffusion models beat gans on image synthesis.
\newblock In {\em Advances in Neural Information Processing Systems}, 2021.

\bibitem[\protect\citeauthoryear{Diao \bgroup \em et al.\egroup
  }{2023}]{diao2023mixture}
Shizhe Diao, Tianyang Xu, Ruijia Xu, Jiawei Wang, and Tong Zhang.
\newblock Mixture-of-domain-adapters: Decoupling and injecting domain knowledge
  to pre-trained language models’ memories.
\newblock In {\em Proceedings of the Annual Meeting of the Association for
  Computational Linguistics}, 2023.

\bibitem[\protect\citeauthoryear{Du and Mordatch}{2019}]{du2019implicit}
Yilun Du and Igor Mordatch.
\newblock Implicit generation and modeling with energy based models.
\newblock In {\em Advances in Neural Information Processing Systems}, 2019.

\bibitem[\protect\citeauthoryear{Elhage \bgroup \em et al.\egroup
  }{2022}]{elhage2022toymodelsof}
Nelson Elhage, Tristan Hume, Catherine Olsson, Nicholas Schiefer, Tom Henighan,
  Shauna Kravec, Zac Hatfield-Dodds, Robert Lasenby, Dawn Drain, Carol Chen,
  et~al.
\newblock Toy models of superposition.
\newblock {\em arXiv preprint arXiv:2209.10652}, 2022.

\bibitem[\protect\citeauthoryear{Geva \bgroup \em et al.\egroup
  }{2021}]{geva-etal-2021-transformer}
Mor Geva, Roei Schuster, Jonathan Berant, and Omer Levy.
\newblock Transformer feed-forward layers are key-value memories.
\newblock In {\em Proceedings of the Conference on Empirical Methods in Natural
  Language Processing}, 2021.

\bibitem[\protect\citeauthoryear{Gong \bgroup \em et al.\egroup
  }{2019}]{gong2019memorizing}
Dong Gong, Lingqiao Liu, Vuong Le, Budhaditya Saha, Moussa~Reda Mansour, Svetha
  Venkatesh, and Anton van~den Hengel.
\newblock Memorizing normality to detect anomaly: Memory-augmented deep
  autoencoder for unsupervised anomaly detection.
\newblock In {\em Proceedings of the IEEE/CVF International Conference on
  Computer Vision}, 2019.

\bibitem[\protect\citeauthoryear{Hacker \bgroup \em et al.\egroup
  }{2023}]{hacker2023regulating}
Philipp Hacker, Andreas Engel, and Marco Mauer.
\newblock Regulating chatgpt and other large generative ai models.
\newblock In {\em Proceedings of the ACM Conference on Fairness,
  Accountability, and Transparency}, 2023.

\bibitem[\protect\citeauthoryear{Ho and Salimans}{2021}]{ho2022classifierfree}
Jonathan Ho and Tim Salimans.
\newblock Classifier-free diffusion guidance.
\newblock In {\em NeurIPS Workshop on Deep Generative Models and Downstream
  Applications}, 2021.

\bibitem[\protect\citeauthoryear{Hu \bgroup \em et al.\egroup
  }{2022}]{hu2021lora}
Edward~J Hu, yelong shen, Phillip Wallis, Zeyuan Allen-Zhu, Yuanzhi Li, Shean
  Wang, Lu~Wang, and Weizhu Chen.
\newblock Lo{RA}: Low-rank adaptation of large language models.
\newblock In {\em International Conference on Learning Representations}, 2022.

\bibitem[\protect\citeauthoryear{Jones \bgroup \em et al.\egroup
  }{1993}]{jones1993lipschitzian}
Donald~R Jones, Cary~D Perttunen, and Bruce~E Stuckman.
\newblock Lipschitzian optimization without the lipschitz constant.
\newblock {\em Journal of optimization Theory and Applications}, 1993.

\bibitem[\protect\citeauthoryear{Khandelwal \bgroup \em et al.\egroup
  }{2020}]{khandelwal2019generalization}
Urvashi Khandelwal, Omer Levy, Dan Jurafsky, Luke Zettlemoyer, and Mike Lewis.
\newblock Generalization through memorization: Nearest neighbor language
  models.
\newblock In {\em International Conference on Learning Representations}, 2020.

\bibitem[\protect\citeauthoryear{Lee \bgroup \em et al.\egroup
  }{2024}]{lee2024gecko}
Jinhyuk Lee, Zhuyun Dai, Xiaoqi Ren, Blair Chen, Daniel Cer, Jeremy~R Cole, Kai
  Hui, Michael Boratko, Rajvi Kapadia, Wen Ding, et~al.
\newblock Gecko: Versatile text embeddings distilled from large language
  models.
\newblock {\em arXiv preprint arXiv:2403.20327}, 2024.

\bibitem[\protect\citeauthoryear{Li \bgroup \em et al.\egroup
  }{2021}]{li2021selfdoc}
Peizhao Li, Jiuxiang Gu, Jason Kuen, Vlad~I Morariu, Handong Zhao, Rajiv Jain,
  Varun Manjunatha, and Hongfu Liu.
\newblock Selfdoc: Self-supervised document representation learning.
\newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition}, 2021.

\bibitem[\protect\citeauthoryear{Lin}{2004}]{lin2004rouge}
Chin-Yew Lin.
\newblock Rouge: A package for automatic evaluation of summaries.
\newblock In {\em Text summarization branches out}, 2004.

\bibitem[\protect\citeauthoryear{Longo \bgroup \em et al.\egroup
  }{2024}]{longo2024explainable}
Luca Longo, Mario Brcic, Federico Cabitza, Jaesik Choi, Roberto Confalonieri,
  Javier Del~Ser, Riccardo Guidotti, Yoichi Hayashi, Francisco Herrera, Andreas
  Holzinger, et~al.
\newblock Explainable artificial intelligence (xai) 2.0: A manifesto of open
  challenges and interdisciplinary research directions.
\newblock {\em Information Fusion}, 2024.

\bibitem[\protect\citeauthoryear{Manakul \bgroup \em et al.\egroup
  }{2023}]{manakul2023selfcheckgpt}
Potsawee Manakul, Adian Liusie, and Mark Gales.
\newblock {S}elf{C}heck{GPT}: Zero-resource black-box hallucination detection
  for generative large language models.
\newblock In {\em Proceedings of the Conference on Empirical Methods in Natural
  Language Processing}, 2023.

\bibitem[\protect\citeauthoryear{Meng \bgroup \em et al.\egroup
  }{2022a}]{meng2023locating}
Kevin Meng, David Bau, Alex Andonian, and Yonatan Belinkov.
\newblock Locating and editing factual associations in gpt.
\newblock In {\em Advances in Neural Information Processing Systems}, 2022.

\bibitem[\protect\citeauthoryear{Meng \bgroup \em et al.\egroup
  }{2022b}]{meng2022mass}
Kevin Meng, Arnab~Sen Sharma, Alex~J Andonian, Yonatan Belinkov, and David Bau.
\newblock Mass-editing memory in a transformer.
\newblock In {\em International Conference on Learning Representations}, 2022.

\bibitem[\protect\citeauthoryear{Merity \bgroup \em et al.\egroup
  }{2017}]{merity2017pointer}
Stephen Merity, Caiming Xiong, James Bradbury, and Richard Socher.
\newblock Pointer sentinel mixture models.
\newblock In {\em International Conference on Learning Representations}, 2017.

\bibitem[\protect\citeauthoryear{Mitchell \bgroup \em et al.\egroup
  }{2023}]{mitchell2023detectgpt}
Eric Mitchell, Yoonho Lee, Alexander Khazatsky, Christopher~D Manning, and
  Chelsea Finn.
\newblock Detectgpt: Zero-shot machine-generated text detection using
  probability curvature.
\newblock In {\em International Conference on Machine Learning}. PMLR, 2023.

\bibitem[\protect\citeauthoryear{Nguyen \bgroup \em et al.\egroup
  }{2023}]{nguyen2023memory}
Dung Nguyen, Phuoc Nguyen, Hung Le, Kien Do, Svetha Venkatesh, and Truyen Tran.
\newblock Memory-augmented theory of mind network.
\newblock In {\em Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2023.

\bibitem[\protect\citeauthoryear{Nichol \bgroup \em et al.\egroup
  }{2022}]{nichol2022glide}
Alexander~Quinn Nichol, Prafulla Dhariwal, Aditya Ramesh, Pranav Shyam, Pamela
  Mishkin, Bob Mcgrew, Ilya Sutskever, and Mark Chen.
\newblock {GLIDE}: Towards photorealistic image generation and editing with
  text-guided diffusion models.
\newblock In {\em Proceedings of the International Conference on Machine
  Learning}. PMLR, 2022.

\bibitem[\protect\citeauthoryear{Pan \bgroup \em et al.\egroup
  }{2020}]{pan2020privacy}
Xudong Pan, Mi~Zhang, Shouling Ji, and Min Yang.
\newblock Privacy risks of general-purpose language models.
\newblock In {\em Proceedings of the IEEE Symposium on Security and Privacy},
  2020.

\bibitem[\protect\citeauthoryear{Reimers and
  Gurevych}{2019}]{reimers2019sentence}
Nils Reimers and Iryna Gurevych.
\newblock Sentence-bert: Sentence embeddings using siamese bert-networks.
\newblock In {\em Proceedings of the Conference on Empirical Methods in Natural
  Language Processing and the International Joint Conference on Natural
  Language Processing}, 2019.

\bibitem[\protect\citeauthoryear{Sallam \bgroup \em et al.\egroup
  }{2023}]{sallam2023chatgpt}
Malik Sallam, Nesreen Salim, Muna Barakat, and Alaa Al-Tammemi.
\newblock Chatgpt applications in medical, dental, pharmacy, and public health
  education: A descriptive study highlighting the advantages and limitations.
\newblock {\em Narra J}, 2023.

\bibitem[\protect\citeauthoryear{Sukhbaatar \bgroup \em et al.\egroup
  }{2015}]{sukhbaatar2015end}
Sainbayar Sukhbaatar, arthur szlam, Jason Weston, and Rob Fergus.
\newblock End-to-end memory networks.
\newblock In {\em Advances in Neural Information Processing Systems}, 2015.

\bibitem[\protect\citeauthoryear{Touvron \bgroup \em et al.\egroup
  }{2023}]{touvron2023llama}
Hugo Touvron, Louis Martin, Kevin Stone, Peter Albert, Amjad Almahairi, Yasmine
  Babaei, Nikolay Bashlykov, Soumya Batra, Prajjwal Bhargava, Shruti Bhosale,
  et~al.
\newblock Llama 2: Open foundation and fine-tuned chat models.
\newblock {\em arXiv preprint arXiv:2307.09288}, 2023.

\bibitem[\protect\citeauthoryear{Wang \bgroup \em et al.\egroup
  }{2022}]{wang2022finding}
Xiaozhi Wang, Kaiyue Wen, Zhengyan Zhang, Lei Hou, Zhiyuan Liu, and Juanzi Li.
\newblock Finding skill neurons in pre-trained transformer-based language
  models.
\newblock In {\em Proceedings of the Conference on Empirical Methods in Natural
  Language Processing}, 2022.

\bibitem[\protect\citeauthoryear{Wu \bgroup \em et al.\egroup
  }{2022}]{wu2022memorizing}
Yuhuai Wu, Markus~Norman Rabe, DeLesley Hutchins, and Christian Szegedy.
\newblock Memorizing transformers.
\newblock In {\em International Conference on Learning Representations}, 2022.

\bibitem[\protect\citeauthoryear{Xie \bgroup \em et al.\egroup
  }{2023}]{xie2023defending}
Yueqi Xie, Jingwei Yi, Jiawei Shao, Justin Curl, Lingjuan Lyu, Qifeng Chen,
  Xing Xie, and Fangzhao Wu.
\newblock Defending chatgpt against jailbreak attack via self-reminders.
\newblock {\em Nature Machine Intelligence}, 2023.

\bibitem[\protect\citeauthoryear{Xu \bgroup \em et al.\egroup
  }{2023}]{pmlr-v202-xu23a}
Frank~F. Xu, Uri Alon, and Graham Neubig.
\newblock Why do nearest neighbor language models work?
\newblock In {\em Proceedings of the International Conference on Machine
  Learning}. PMLR, 2023.

\bibitem[\protect\citeauthoryear{Yao \bgroup \em et al.\egroup
  }{2023}]{yao2023editing}
Yunzhi Yao, Peng Wang, Bozhong Tian, Siyuan Cheng, Zhoubo Li, Shumin Deng,
  Huajun Chen, and Ningyu Zhang.
\newblock Editing large language models: Problems, methods, and opportunities.
\newblock In {\em Proceedings of the Conference on Empirical Methods in Natural
  Language Processing}, 2023.

\bibitem[\protect\citeauthoryear{Yu \bgroup \em et al.\egroup
  }{2023}]{yu2023codeipprompt}
Zhiyuan Yu, Yuhao Wu, Ning Zhang, Chenguang Wang, Yevgeniy Vorobeychik, and
  Chaowei Xiao.
\newblock Codeipprompt: intellectual property infringement assessment of code
  language models.
\newblock In {\em Proceedings of the International Conference on Machine
  Learning}. PMLR, 2023.

\end{thebibliography}

